Where Does the Robustness Come from? A Study of the Transformation-based Ensemble Defence

This paper aims to provide a thorough study on the effectiveness of the transformation-based ensemble defence for image classification and its reasons. It has been empirically shown that they can enhance the robustness against evasion attacks, while there is little analysis on the reasons. In particular, it is not clear whether the robustness improvement is a result of transformation or ensemble. In this paper, we design two adaptive attacks to better evaluate the transformation-based ensemble defence. We conduct experiments to show that 1) the transferability of adversarial examples exists among the models trained on data records after different reversible transformations; 2) the robustness gained through transformation-based ensemble is limited; 3) this limited robustness is mainly from the irreversible transformations rather than the ensemble of a number of models; and 4) blindly increasing the number of sub-models in a transformation-based ensemble does not bring extra robustness gain.

==> experiment.tex <==
\subsection{Experiment Setup}\label{subsec:experiment-setup}

\begin{table*}[]
\centering
\caption{Classification Accuracy of ATHENA Ensemble under Adaptive Attacks on MNIST}
\label{tab:mnist_attack_result}
\resizebox{1.2\columnwidth}{!}{%
\begin{tabular}{|c|c|c|c|c|c|c|}
\hline
\multicolumn{2}{|l|}{} & \textbf{RD} & \textbf{MV} & \textbf{T2MV} & \textbf{AP} & \textbf{AL} \\ \hline
\multicolumn{2}{|c|}{\textbf{Benign}} & 0.9958 & 0.9968 & 0.9945 & 0.9968 & 0.9968 \\ \hline
\multirow{5}{*}{\textbf{FGSM}} & \textit{\textbf{Original}} & 0.98 & 0.9933 & 0.9767 & 0.9945 & 0.9945 \\ \cline{2-7}
 & \textit{\textbf{Transformed}} & 0.7664 & 0.8028 & 0.7968 & 0.819 & 0.832 \\ \cline{2-7}
 & \textit{\textbf{Overall TR}} & 0.6242 & 0.5986 & 0.6076 & 0.6314 & 0.7298 \\ \cline{2-7}
 & \textit{\textbf{Label-wise TR}} & 0.3072 & 0.318 & 0.3216 & 0.371 & 0.4902 \\ \cline{2-7}
 & \textit{\textbf{Individual TR}} & 0.33 & 0.33 & 0.33 & 0.33 & 0.36 \\ \hline
\multirow{5}{*}{\textbf{PGD}} & \textit{\textbf{Original}} & 0.9934 & 0.9966 & 0.9926 & 0.99964 & 0.9966 \\ \cline{2-7}
 & \textit{\textbf{Transformed}} & 0.8982 & 0.919 & 0.9118 & 0.9184 & 0.9198 \\ \cline{2-7}
 & \textit{\textbf{Overall TR}} & 0.9908 & 0.9966 & 0.9908 & 0.9966 & 0.9968 \\ \cline{2-7}
 & \textit{\textbf{Label-wise TR}} & 0.944 & 0.9574 & 0.956 & 0.958 & 0.9584 \\ \cline{2-7}
 & \textit{\textbf{Individual TR}} & 0.89 & 0.89 & 0.89 & 0.89 & 0.89 \\ \hline
\multirow{5}{*}{\textbf{C\&W}} & \textit{\textbf{Original}} & 0.9878 & 0.9942 & 0.9904 & 0.994 & 0.994 \\ \cline{2-7}
 & \textit{\textbf{Transformed}} & 0.9232 & 0.919 & 0.9176 & 0.9254 & 0.9348 \\ \cline{2-7}
 & \textit{\textbf{Overall TR}} & 0.939 & 0.947 & 0.9454 & 0.95 & 0.963 \\ \cline{2-7}
 & \textit{\textbf{Label-wise TR}} & 0.7026 & 0.6322 & 0.6382 & 0.6592 & 0.7136 \\ \cline{2-7}
 & \textit{\textbf{Individual TR}} & 0.85 & 0.85 & 0.85 & 0.85 & 0.85 \\ \hline
\multirow{5}{*}{\textbf{DeepFool}} & \textit{\textbf{Original}} & 0.991 & 0.9954 & 0.993 & 0.9954 & 0.9952 \\ \cline{2-7}
 & \textit{\textbf{Transformed}} & 0.8734 & 0.8994 & 0.897 & 0.9068 & 0.9202 \\ \cline{2-7}
 & \textit{\textbf{Overall TR}} & 0.9228 & 0.9214 & 0.9214 & 0.9268 & 0.9436 \\ \cline{2-7}
 & \textit{\textbf{Label-wise TR}} & 0.5136 & 0.5252 & 0.5298 & 0.5484 & 0.618 \\ \cline{2-7}
 & \textit{\textbf{Individual TR}} & 0.74 & 0.79 & 0.78 & 0.79 & 0.79 \\ \hline
\end{tabular}%
}
\end{table*}

\begin{table*}[]
\centering
\caption{Transferability Rate of Adversarial Examples Generated on Different Ensemble Members}
\label{tab:trans_result_mnist}
\resizebox{\textwidth}{!}{%
\begin{tabular}{|c|c|c|c|c|c|c|c|c|c|c|c|c|c|c|c|c|c|c|c|}
\hline
\textbf{Dataset} & \textbf{transformation} & \textbf{\begin{tabular}[c]{@{}c@{}}attack\\ method\end{tabular}} & \textbf{\begin{tabular}[c]{@{}c@{}}number\\ of\\  AEs\end{tabular}} & \textbf{cur} & \textbf{\begin{tabular}[c]{@{}c@{}}flip\\ both\end{tabular}} & \textbf{\begin{tabular}[c]{@{}c@{}}flip\\ horizontal\end{tabular}} & \textbf{\begin{tabular}[c]{@{}c@{}}flip\\ vertical\end{tabular}} & \textbf{\begin{tabular}[c]{@{}c@{}}rotate\\ 180\end{tabular}} & \textbf{\begin{tabular}[c]{@{}c@{}}rotate\\ 270\end{tabular}} & \textbf{\begin{tabular}[c]{@{}c@{}}rotate\\ 90\end{tabular}} & \textbf{\begin{tabular}[c]{@{}c@{}}shift\\ bottom\\ left\end{tabular}} & \textbf{\begin{tabular}[c]{@{}c@{}}shift\\ bottom\\ right\end{tabular}} & \textbf{\begin{tabular}[c]{@{}c@{}}shift\\ down\end{tabular}} & \textbf{\begin{tabular}[c]{@{}c@{}}shift\\ left\end{tabular}} & \textbf{\begin{tabular}[c]{@{}c@{}}shift\\ right\end{tabular}} & \textbf{\begin{tabular}[c]{@{}c@{}}shift\\ top\\ left\end{tabular}} & \textbf{\begin{tabular}[c]{@{}c@{}}shift\\ top\\ right\end{tabular}} & \textbf{\begin{tabular}[c]{@{}c@{}}shift\\ up\end{tabular}} & \textbf{Average} \\ \hline
\multirow{56}{*}{\textbf{MNIST}} & \multirow{4}{*}{\textbf{\begin{tabular}[c]{@{}c@{}}flip\\ both\end{tabular}}} & \textbf{FGSM} & 43 & 100.00\% & 100.00\% & 57.14\% & 52.54\% & 37.33\% & 31.75\% & 41.18\% & 40.70\% & 34.94\% & 40.91\% & 48.28\% & 50.00\% & 19.28\% & 35.80\% & 32.31\% & 62.78\% \\ \cline{3-20} 
 &  & \textbf{PGD} & 100 & 100.00\% & 100.00\% & 71.00\% & 65.66\% & 58.00\% & 44.00\% & 67.00\% & 64.00\% & 53.00\% & 57.00\% & 66.00\% & 59.18\% & 30.00\% & 57.00\% & 39.00\% & 69.64\% \\ \cline{3-20} 
 &  & \textbf{C\&W} & 52 & 100.00\% & 100.00\% & 8.96\% & 4.08\% & 8.33\% & 2.50\% & 2.82\% & 17.39\% & 12.50\% & 7.69\% & 14.93\% & 14.06\% & 3.45\% & 7.27\% & 8.51\% & 12.91\% \\ \cline{3-20} 
 &  & \textbf{DeepFool} & 54 & 100.00\% & 100.00\% & 0.00\% & 1.79\% & 0.00\% & 0.00\% & 3.51\% & 1.96\% & 0.00\% & 3.33\% & 1.72\% & 4.08\% & 1.82\% & 3.70\% & 0.00\% & 7.94\% \\ \cline{2-20} 
 & \multirow{4}{*}{\textbf{\begin{tabular}[c]{@{}c@{}}flip\\ horizontal\end{tabular}}} & \textbf{FGSM} & 35 & 100.00\% & 57.89\% & 100.00\% & 54.24\% & 41.33\% & 20.63\% & 39.71\% & 40.70\% & 33.73\% & 39.39\% & 50.00\% & 54.69\% & 19.28\% & 35.80\% & 23.08\% & 57.60\% \\ \cline{3-20} 
 &  & \textbf{PGD} & 69 & 100.00\% & 69.00\% & 100.00\% & 67.68\% & 56.00\% & 36.00\% & 77.00\% & 65.00\% & 59.00\% & 64.00\% & 71.00\% & 76.53\% & 37.00\% & 53.00\% & 58.00\% & 70.07\% \\ \cline{3-20} 
 &  & \textbf{C\&W} & 67 & 100.00\% & 3.85\% & 100.00\% & 6.12\% & 6.67\% & 2.50\% & 4.23\% & 6.52\% & 10.42\% & 7.69\% & 13.43\% & 14.06\% & 6.90\% & 9.09\% & 14.89\% & 12.26\% \\ \cline{3-20} 
 &  & \textbf{DeepFool} & 54 & 100.00\% & 0.00\% & 100.00\% & 1.79\% & 1.72\% & 0.00\% & 0.00\% & 1.96\% & 0.00\% & 5.00\% & 5.17\% & 4.08\% & 0.00\% & 1.85\% & 0.00\% & 8.33\% \\ \cline{2-20} 
 & \multirow{4}{*}{\textbf{\begin{tabular}[c]{@{}c@{}}flip\\ vertical\end{tabular}}} & \textbf{FGSM} & 40 & 100.00\% & 63.16\% & 57.14\% & 100.00\% & 36.00\% & 34.92\% & 45.59\% & 54.65\% & 44.58\% & 63.64\% & 53.45\% & 54.69\% & 21.69\% & 43.21\% & 24.62\% & 56.30\% \\ \cline{3-20} 
 &  & \textbf{PGD} & 81 & 100.00\% & 81.00\% & 72.00\% & 100.00\% & 50.00\% & 48.00\% & 70.00\% & 70.00\% & 57.00\% & 66.00\% & 73.00\% & 63.27\% & 35.00\% & 57.00\% & 54.00\% & 63.78\% \\ \cline{3-20} 
 &  & \textbf{C\&W} & 49 & 100.00\% & 1.92\% & 4.48\% & 100.00\% & 5.00\% & 10.00\% & 2.82\% & 6.52\% & 10.42\% & 6.15\% & 7.46\% & 10.94\% & 6.90\% & 12.73\% & 6.38\% & 11.22\% \\ \cline{3-20} 
 &  & \textbf{DeepFool} & 56 & 100.00\% & 0.00\% & 1.85\% & 100.00\% & 0.00\% & 0.00\% & 0.00\% & 1.96\% & 3.33\% & 6.67\% & 3.45\% & 12.24\% & 1.82\% & 7.41\% & 0.00\% & 8.67\% \\ \cline{2-20} 
 & \multirow{4}{*}{\textbf{rotate 180}} & \textbf{FGSM} & 23 & 100.00\% & 49.12\% & 52.38\% & 45.76\% & 100.00\% & 31.75\% & 41.18\% & 51.16\% & 32.53\% & 45.45\% & 51.72\% & 65.62\% & 27.71\% & 39.51\% & 40.00\% & 45.81\% \\ \cline{3-20} 
 &  & \textbf{PGD} & 71 & 100.00\% & 71.00\% & 64.00\% & 61.62\% & 100.00\% & 49.00\% & 57.00\% & 60.00\% & 47.00\% & 54.00\% & 57.00\% & 53.06\% & 35.00\% & 57.00\% & 54.00\% & 57.50\% \\ \cline{3-20} 
 &  & \textbf{C\&W} & 60 & 100.00\% & 5.77\% & 4.48\% & 0.00\% & 100.00\% & 2.50\% & 4.23\% & 8.70\% & 12.50\% & 7.69\% & 4.48\% & 7.81\% & 0.00\% & 5.45\% & 6.38\% & 12.26\% \\ \cline{3-20} 
 &  & \textbf{DeepFool} & 58 & 100.00\% & 0.00\% & 0.00\% & 1.79\% & 100.00\% & 0.00\% & 1.75\% & 1.96\% & 0.00\% & 5.00\% & 0.00\% & 6.12\% & 0.00\% & 0.00\% & 0.00\% & 8.13\% \\ \cline{2-20} 
 & \multirow{4}{*}{\textbf{rotate 270}} & \textbf{FGSM} & 37 & 100.00\% & 61.40\% & 49.21\% & 49.15\% & 41.33\% & 100.00\% & 42.65\% & 50.00\% & 37.35\% & 57.58\% & 39.66\% & 57.81\% & 24.10\% & 43.21\% & 33.85\% & 37.07\% \\ \cline{3-20} 
 &  & \textbf{PGD} & 77 & 100.00\% & 77.00\% & 71.00\% & 59.60\% & 76.00\% & 100.00\% & 59.00\% & 69.00\% & 62.00\% & 67.00\% & 68.00\% & 63.27\% & 42.00\% & 61.00\% & 71.00\% & 44.64\% \\ \cline{3-20} 
 &  & \textbf{C\&W} & 40 & 100.00\% & 7.69\% & 2.99\% & 2.04\% & 8.33\% & 100.00\% & 1.41\% & 8.70\% & 2.08\% & 9.23\% & 7.46\% & 9.38\% & 3.45\% & 7.27\% & 10.64\% & 10.89\% \\ \cline{3-20} 
 &  & \textbf{DeepFool} & 61 & 100.00\% & 1.85\% & 5.56\% & 1.79\% & 5.17\% & 100.00\% & 0.00\% & 5.88\% & 3.33\% & 5.00\% & 3.45\% & 8.16\% & 1.82\% & 7.41\% & 3.70\% & 7.14\% \\ \cline{2-20} 
 & \multirow{4}{*}{\textbf{rotate 90}} & \textbf{FGSM} & 32 & 100.00\% & 59.65\% & 52.38\% & 62.71\% & 42.67\% & 26.98\% & 100.00\% & 44.19\% & 34.94\% & 43.94\% & 44.83\% & 53.12\% & 19.28\% & 35.80\% & 21.54\% & 50.11\% \\ \cline{3-20} 
 &  & \textbf{PGD} & 62 & 100.00\% & 62.00\% & 79.00\% & 60.61\% & 57.00\% & 32.00\% & 100.00\% & 65.00\% & 57.00\% & 64.00\% & 73.00\% & 63.27\% & 45.00\% & 51.00\% & 51.00\% & 66.14\% \\ \cline{3-20} 
 &  & \textbf{C\&W} & 71 & 100.00\% & 5.77\% & 4.48\% & 6.12\% & 6.67\% & 0.00\% & 100.00\% & 4.35\% & 10.42\% & 6.15\% & 10.45\% & 10.94\% & 0.00\% & 5.45\% & 8.51\% & 9.76\% \\ \cline{3-20} 
 &  & \textbf{DeepFool} & 57 & 100.00\% & 0.00\% & 0.00\% & 1.79\% & 0.00\% & 0.00\% & 100.00\% & 0.00\% & 1.67\% & 1.67\% & 0.00\% & 2.04\% & 0.00\% & 0.00\% & 0.00\% & 8.02\% \\ \cline{2-20} 
 & \multirow{4}{*}{\textbf{\begin{tabular}[c]{@{}c@{}}shift\\ bottom\\ left\end{tabular}}} & \textbf{FGSM} & 14 & 100.00\% & 73.68\% & 63.49\% & 52.54\% & 44.00\% & 23.81\% & 55.88\% & 100.00\% & 48.19\% & 75.76\% & 60.34\% & 64.06\% & 25.30\% & 46.91\% & 32.31\% & 54.73\% \\ \cline{3-20} 
 &  & \textbf{PGD} & 57 & 100.00\% & 57.00\% & 59.00\% & 50.51\% & 45.00\% & 35.00\% & 67.00\% & 100.00\% & 62.00\% & 77.00\% & 62.00\% & 56.12\% & 38.00\% & 47.00\% & 33.00\% & 67.57\% \\ \cline{3-20} 
 &  & \textbf{C\&W} & 46 & 100.00\% & 11.54\% & 7.46\% & 4.08\% & 5.00\% & 7.50\% & 1.41\% & 100.00\% & 10.42\% & 12.31\% & 10.45\% & 14.06\% & 0.00\% & 3.64\% & 8.51\% & 14.75\% \\ \cline{3-20} 
 &  & \textbf{DeepFool} & 51 & 100.00\% & 0.00\% & 0.00\% & 1.79\% & 0.00\% & 0.00\% & 0.00\% & 100.00\% & 0.00\% & 6.67\% & 3.45\% & 4.08\% & 0.00\% & 0.00\% & 0.00\% & 9.52\% \\ \cline{2-20} 
 & \multirow{4}{*}{\textbf{\begin{tabular}[c]{@{}c@{}}shift\\ bottom\\ right\end{tabular}}} & \textbf{FGSM} & 19 & 100.00\% & 52.63\% & 46.03\% & 54.24\% & 33.33\% & 25.40\% & 50.00\% & 55.81\% & 100.00\% & 62.12\% & 48.28\% & 73.44\% & 8.43\% & 51.85\% & 20.00\% & 44.32\% \\ \cline{3-20} 
 &  & \textbf{PGD} & 52 & 100.00\% & 52.00\% & 54.00\% & 51.52\% & 36.00\% & 32.00\% & 56.00\% & 63.00\% & 100.00\% & 71.00\% & 54.00\% & 66.33\% & 27.00\% & 59.00\% & 38.00\% & 61.86\% \\ \cline{3-20} 
 &  & \textbf{C\&W} & 48 & 100.00\% & 1.92\% & 1.49\% & 0.00\% & 0.00\% & 0.00\% & 1.41\% & 6.52\% & 100.00\% & 4.62\% & 1.49\% & 6.25\% & 0.00\% & 5.45\% & 2.13\% & 15.62\% \\ \cline{3-20} 
 &  & \textbf{DeepFool} & 60 & 100.00\% & 0.00\% & 1.85\% & 1.79\% & 0.00\% & 0.00\% & 1.75\% & 1.96\% & 100.00\% & 1.67\% & 3.45\% & 6.12\% & 0.00\% & 5.56\% & 0.00\% & 8.81\% \\ \cline{2-20} 
 & \multirow{4}{*}{\textbf{\begin{tabular}[c]{@{}c@{}}shift\\ down\end{tabular}}} & \textbf{FGSM} & 35 & 100.00\% & 43.86\% & 41.27\% & 49.15\% & 34.67\% & 22.22\% & 45.59\% & 58.14\% & 43.37\% & 100.00\% & 56.90\% & 60.94\% & 14.46\% & 29.63\% & 20.00\% & 56.71\% \\ \cline{3-20} 
 &  & \textbf{PGD} & 56 & 100.00\% & 56.00\% & 67.00\% & 59.60\% & 50.00\% & 31.00\% & 61.00\% & 72.00\% & 75.00\% & 100.00\% & 70.00\% & 65.31\% & 25.00\% & 55.00\% & 47.00\% & 67.07\% \\ \cline{3-20} 
 &  & \textbf{C\&W} & 65 & 100.00\% & 5.77\% & 1.49\% & 2.04\% & 1.67\% & 7.50\% & 1.41\% & 6.52\% & 8.33\% & 100.00\% & 1.49\% & 4.69\% & 0.00\% & 0.00\% & 2.13\% & 14.29\% \\ \cline{3-20} 
 &  & \textbf{DeepFool} & 60 & 100.00\% & 3.70\% & 0.00\% & 1.79\% & 0.00\% & 0.00\% & 0.00\% & 0.00\% & 3.33\% & 100.00\% & 1.72\% & 4.08\% & 0.00\% & 1.85\% & 0.00\% & 10.71\% \\ \cline{2-20} 
 & \multirow{4}{*}{\textbf{\begin{tabular}[c]{@{}c@{}}shift\\ left\end{tabular}}} & \textbf{FGSM} & 39 & 100.00\% & 49.12\% & 47.62\% & 49.15\% & 21.33\% & 23.81\% & 36.76\% & 50.00\% & 26.51\% & 37.88\% & 100.00\% & 48.44\% & 10.84\% & 38.27\% & 23.08\% & 58.25\% \\ \cline{3-20} 
 &  & \textbf{PGD} & 79 & 100.00\% & 79.00\% & 77.00\% & 66.67\% & 52.00\% & 38.00\% & 76.00\% & 69.00\% & 55.00\% & 68.00\% & 100.00\% & 73.47\% & 30.00\% & 51.00\% & 43.00\% & 68.14\% \\ \cline{3-20} 
 &  & \textbf{C\&W} & 67 & 100.00\% & 7.69\% & 7.46\% & 10.20\% & 3.33\% & 2.50\% & 7.04\% & 8.70\% & 10.42\% & 10.77\% & 100.00\% & 12.50\% & 3.45\% & 7.27\% & 6.38\% & 13.75\% \\ \cline{3-20} 
 &  & \textbf{DeepFool} & 58 & 100.00\% & 0.00\% & 1.85\% & 3.57\% & 1.72\% & 0.00\% & 0.00\% & 5.88\% & 5.00\% & 3.33\% & 100.00\% & 4.08\% & 0.00\% & 5.56\% & 1.85\% & 9.61\% \\ \cline{2-20} 
 & \multirow{4}{*}{\textbf{\begin{tabular}[c]{@{}c@{}}shift\\ right\end{tabular}}} & \textbf{FGSM} & 34 & 100.00\% & 45.61\% & 53.97\% & 50.85\% & 38.67\% & 34.92\% & 36.76\% & 44.19\% & 43.37\% & 48.48\% & 51.72\% & 100.00\% & 20.48\% & 50.62\% & 35.38\% & 65.18\% \\ \cline{3-20} 
 &  & \textbf{PGD} & 54 & 100.00\% & 54.00\% & 59.00\% & 51.52\% & 40.00\% & 33.00\% & 43.00\% & 53.00\% & 58.00\% & 55.00\% & 59.00\% & 100.00\% & 28.00\% & 60.00\% & 42.00\% & 68.73\% \\ \cline{3-20} 
 &  & \textbf{C\&W} & 64 & 100.00\% & 3.85\% & 2.99\% & 6.12\% & 8.33\% & 5.00\% & 1.41\% & 8.70\% & 4.17\% & 6.15\% & 4.48\% & 100.00\% & 0.00\% & 5.45\% & 6.38\% & 17.41\% \\ \cline{3-20} 
 &  & \textbf{DeepFool} & 49 & 100.00\% & 0.00\% & 0.00\% & 1.79\% & 1.72\% & 0.00\% & 0.00\% & 1.96\% & 0.00\% & 3.33\% & 1.72\% & 100.00\% & 0.00\% & 0.00\% & 1.85\% & 13.12\% \\ \cline{2-20} 
 & \multirow{4}{*}{\textbf{\begin{tabular}[c]{@{}c@{}}shift\\ top left\end{tabular}}} & \textbf{FGSM} & 19 & 100.00\% & 101.75\% & 90.48\% & 76.27\% & 78.67\% & 66.67\% & 77.94\% & 74.42\% & 55.42\% & 75.76\% & 100.00\% & 93.75\% & 100.00\% & 74.07\% & 66.15\% & 25.73\% \\ \cline{3-20} 
 &  & \textbf{PGD} & 80 & 100.00\% & 80.00\% & 78.00\% & 75.76\% & 73.00\% & 58.00\% & 74.00\% & 76.00\% & 64.00\% & 69.00\% & 80.00\% & 75.51\% & 100.00\% & 79.00\% & 79.00\% & 39.57\% \\ \cline{3-20} 
 &  & \textbf{C\&W} & 29 & 100.00\% & 3.85\% & 7.46\% & 4.08\% & 6.67\% & 5.00\% & 1.41\% & 10.87\% & 8.33\% & 6.15\% & 10.45\% & 14.06\% & 100.00\% & 10.91\% & 12.77\% & 9.36\% \\ \cline{3-20} 
 &  & \textbf{DeepFool} & 55 & 100.00\% & 3.70\% & 1.85\% & 1.79\% & 3.45\% & 0.00\% & 5.26\% & 5.88\% & 3.33\% & 3.33\% & 6.90\% & 16.33\% & 100.00\% & 7.41\% & 3.70\% & 7.53\% \\ \cline{2-20} 
 & \multirow{4}{*}{\textbf{\begin{tabular}[c]{@{}c@{}}shift\\ top right\end{tabular}}} & \textbf{FGSM} & 21 & 100.00\% & 68.42\% & 49.21\% & 50.85\% & 46.67\% & 42.86\% & 44.12\% & 48.84\% & 48.19\% & 56.06\% & 60.34\% & 73.44\% & 30.12\% & 100.00\% & 44.62\% & 47.44\% \\ \cline{3-20} 
 &  & \textbf{PGD} & 71 & 100.00\% & 71.00\% & 57.00\% & 58.59\% & 51.00\% & 35.00\% & 50.00\% & 62.00\% & 62.00\% & 59.00\% & 60.00\% & 77.55\% & 37.00\% & 100.00\% & 47.00\% & 61.00\% \\ \cline{3-20} 
 &  & \textbf{C\&W} & 55 & 100.00\% & 11.54\% & 8.96\% & 4.08\% & 5.00\% & 2.50\% & 2.82\% & 4.35\% & 8.33\% & 7.69\% & 1.49\% & 10.94\% & 3.45\% & 100.00\% & 6.38\% & 13.51\% \\ \cline{3-20} 
 &  & \textbf{DeepFool} & 54 & 100.00\% & 0.00\% & 0.00\% & 0.00\% & 0.00\% & 0.00\% & 0.00\% & 0.00\% & 1.67\% & 0.00\% & 1.72\% & 4.08\% & 0.00\% & 100.00\% & 0.00\% & 10.32\% \\ \cline{2-20} 
 & \multirow{4}{*}{\textbf{shift up}} & \textbf{FGSM} & 35 & 100.00\% & 52.63\% & 46.03\% & 40.68\% & 45.33\% & 33.33\% & 44.12\% & 53.49\% & 37.35\% & 46.97\% & 50.00\% & 62.50\% & 19.28\% & 39.51\% & 100.00\% & 36.92\% \\ \cline{3-20} 
 &  & \textbf{PGD} & 66 & 100.00\% & 66.00\% & 73.00\% & 63.64\% & 61.00\% & 54.00\% & 69.00\% & 58.00\% & 55.00\% & 68.00\% & 61.00\% & 69.39\% & 45.00\% & 67.00\% & 100.00\% & 54.00\% \\ \cline{3-20} 
 &  & \textbf{C\&W} & 47 & 100.00\% & 9.62\% & 8.96\% & 8.16\% & 6.67\% & 5.00\% & 4.23\% & 8.70\% & 10.42\% & 7.69\% & 4.48\% & 14.06\% & 3.45\% & 9.09\% & 100.00\% & 14.29\% \\ \cline{3-20} 
 &  & \textbf{DeepFool} & 54 & 100.00\% & 1.85\% & 3.70\% & 0.00\% & 0.00\% & 0.00\% & 0.00\% & 3.92\% & 1.67\% & 5.00\% & 1.72\% & 8.16\% & 0.00\% & 3.70\% & 100.00\% & 7.94\% \\ \hline
\end{tabular}%
}
\end{table*}

In line with white box or gray box setting in~\cite{meng2020ensembles},
we evaluated our attack algorithm on MNIST dataset.
It contains 70000 gray-scale images of hand-written digits, we split the dataset into three small sets: training,
testing and validation at the ratio of 12:1:1.
Unlike training procedure in~\cite{meng2020ensembles}, early-stopping technique based on cross-entropy loss on
validation dataset was adopted to prevent models from over-fitting in our case.

As for our target models, we adopt the settings in~\cite{meng2020ensembles}.
The model structure is shown in Fig.~\ref{fig: mnist_model_structure}.
These 73 ensemble members are trained on the same set of examples but with different transformations and the final
prediction is generated on the output of those ensemble members in 5 ensemble strategies: Random Defense (RD),
Majority Voting (MV), Top 2 Majority Voting (T2MV), Average Probabilities (AP), Average Logits (AL).

\begin{figure}[b]
    \centering
    \includegraphics[width=\columnwidth]{figures/mnist/mnist_model_structure.png}
    \caption{Structure of target model on MNIST dataset}
    \label{fig: mnist_model_structure}
\end{figure}

\begin{table}[b]
\centering
\caption{Parameters for attack algorithms}
\label{tab:attack_params}
\resizebox{0.7\columnwidth}{!}{%
\begin{tabular}{|c|c|}
\hline
\textbf{\begin{tabular}[c]{@{}c@{}}Attack\\ Algorithm\end{tabular}} & \textbf{Parameters} \\ \hline
\textbf{FGSM} & \begin{tabular}[c]{@{}c@{}}norm=$\infty$\\ eps=0.1\end{tabular} \\ \hline
\textbf{PGD} & \begin{tabular}[c]{@{}c@{}}norm=$\infty$,\\ eps=0.05,\\ maximum iterations=250\end{tabular} \\ \hline
\textbf{C\&W} & \begin{tabular}[c]{@{}c@{}}norm=2\\ binary search steps=10,\\ initial constant=10,\\ learning rate=0.1.\\ maximum iteration=100\end{tabular} \\ \hline
\textbf{DeepFool} & \begin{tabular}[c]{@{}c@{}}norm=2,\\ maximum iteration=100,\\ overshoot=1,\\ number of candidates=3\end{tabular} \\ \hline
\end{tabular}%
}
\end{table}

While~\cite{meng2020ensembles} only applied their attack algorithm with Fast Gradient Sign Method(FGSM),
we extended the list of attacker to gradient based attackers includes Fast Gradient Sign Method (FGSM), Projected
Gradient Descent (PGD), DeepFool and Carlini\& Wagner's $l_2$ norm bounded attack (C\&W).
In following sections, we'll refer those abbreviations to their settings as in Table.~\ref{tab:attack_params} if not
specified.
Due to the similar iterative nature between Basic Iterative Method, Momentum Iterative Method and
Projected Gradient Descent, only Projected Gradient Descent is evaluated in our experiments since it
has higher success rate on MNIST dataset as pointed out in~\cite{carlini2017towards}.
Also, to ensure our attacker has found the optimised adversarial perturbation, the parameters for our iteration-based or
optimisation-based attacks are set in an overkill way as in~\ref{tab:attack_params}.
As for the knowledge of adversary, we expose our ensemble under the worst-case scenario where the adversary has full
knowledge about the ensemble but we assume the attacker is greedy that it won't stop updating the adversarial
perturbation until exceeding preset budget.
All the attack algorithms mentioned above are using Adversarial Robustness Toolbox's implementation and ensemble
members are using PyTorch framework.

For each attack, we conducted our adaptive attack experiment in several settings: defence evaluation under original
setting as in~\cite{athena}, we denote this scenario as \textit{original};
defence evaluation with adversarial perturbations generated on transformed input, we denote is as \textit{Transformed};
defence evaluation under our adaptive attack scenario with three different approaches for transferability ranking as
in~\ref{subsec:adaptive-attack} and we denote those attacks with their corresponding transferability ranking method as
\textit{Individual TR}, \textit{Overall TR}, \textit{Label-wise TR}.
For our proposed defense method, we denote the distilled ensemble with $N$ ensemble members as \textit{$N$-limited} and
we put it under our adaptive attack in \textit{Label-wise TR} and \textit{Overall TR} fashion.

\subsection{Transferability Results}\label{subsec:transferability-results}

In this paper, transferability of certain ensemble member is evaluated and quantified
based on the number of all the ensemble members fooled by attacking on it, i.e.\ transferability $T\in[0, n]$
where $n$ is the total number of ensemble members.
Due to the large number of examples, it is computationally expensive to run transferability as described in
section~\ref{subsubsec:individual-ranking-based}.

\subsubsection{Correlation for dataset-wise transferability rankings}
To use the transferability ranking generated on a set with fewer examples as the approximation for all 5000 examples in
test dataset, we evaluated the correlation coefficient between average transferability rankings generated on different
sets of examples with FGSM attack.
Correlation result for this set of comparison is shown in Fig~\ref{fig:sample_trans_coeff}, where the correlation
coefficient between transferability ranking generated on 100 examples and the one generated on 3000 examples are as high
as 0.9936, hence they can be regarded as highly related and our approximation for overall transferability ranking with
the one generated on randomly chosen examples is valid.

\begin{figure}[t]
    \centering
    \caption{Correlation of transferability generated on different number of samples}
    \includegraphics[width=.7\columnwidth]{figures/mnist/sample_trans_coeff.png}
    \label{fig:sample_trans_coeff}
\end{figure}

\subsubsection{Correlation for attack-wise transferability rankings}
Furthermore, to use transferability ranking generated with faster attack algorithms as FGSM as approximation for those
generated with other attack algorithms, we evaluated the correlation coefficient between transferability ranking
generated on 100 randomly chosen examples with FGSM, PGD, C\&W and DeepFool attacks.
The result is illustrated in Fig~\ref{fig:attack_trans_coeff}.
Similar to the result in Fig~\ref{fig:sample_trans_coeff}, the ranking correlation between transferability ranking
generated with different attacks is also so close to 1 that our approximation also stands.

\begin{figure}[t]
    \centering
    \caption{Correlation of transferability generated with different attacks}
    \includegraphics[width=.7\columnwidth]{figures/mnist/attack_trans_coeff.png}
    \label{fig:attack_trans_coeff}
\end{figure}

As indicated by the figures, the correlation between transferability ranking under different settings are very close
to 1, which means the transferability ranking for certain ensemble member is highly similar.
This proves that the transferability of certain model is the nature of the model instead of nature of attack
algorithm or nature of examples.

\subsubsection{Correlation for label-wise transferability rankings}
Also, we evaluate the correlation coefficient between transferability rankings generated on examples from different
classes as mentioned in section~\ref{subsubsec:average-ranking-over-classes}.
Based on previous assumptions, we use the label-wise transferability rankings generated on the 100 randomly chosen
examples with FGSM and the result is shown in Fig.~\ref{fig:label_trans_coeff}.

\begin{figure}[t]
    \centering
    \caption{Correlation of transferability generated on examples from different classes}
    \includegraphics[width=.7\columnwidth]{figures/mnist/label_trans_coeff.png}
    \label{fig:label_trans_coeff}
\end{figure}

Different from our previous experiments on transferability rankings, the correlation matrix of label-wise
transferability ranking shows lower similarity and it means that adaptive attack with \textit{Overall TR} might not be
appropriate and it is proved in Table.~\ref{tab:mnist_attack_result} in the relatively higher classification accuracy on generated
adversarial examples.

With this in mind, one may wonder that the effects of different attacks on examples from different classes may differs.
Hence, we calculated correlation correlation coefficient between transferability rankings generated on examples from
diverse classes with FGSM, PGD, C\&W and DeepFool in Fig.~\ref{fig:attack_trans_coeff_label}.
It supports our previous assumptions that transferability rankings generated with different attacks are similar to each
other no matter the ground truth label for the example it generated on.
Hence, it is reasonable for us to perform adaptive attacks using \textit{Label-wise TR} generated with FGSM\@. \\

%\begin{figure}[t]
%    \centering
%    \begin{subfigure}
%%        \captionsetup{width=.18\linewidth}
%%        \caption{Correlation of transferability generated with different attacks on examples with ground truth label 0}
%        \includegraphics[width=.4\linewidth]{figures/mnist/attack_trans_coeff_label_0.png}
%        \caption{\label{fig:label 0 }}
%    \end{subfigure}
%    \begin{subfigure}
%        \includegraphics[width=.4\linewidth]{figures/mnist/attack_trans_coeff_label_1.png}
%%        \caption{Correlation of transferability generated with different attacks on examples with ground truth label 1}
%    \end{subfigure}
%    \begin{subfigure}
%        \includegraphics[width=.4\linewidth]{figures/mnist/attack_trans_coeff_label_2.png}
%%        \caption{Correlation of transferability generated with different attacks on examples with ground truth label 2}
%    \end{subfigure}
%    \begin{subfigure}
%        \includegraphics[width=.4\linewidth]{figures/mnist/attack_trans_coeff_label_3.png}
%%        \caption{Correlation of transferability generated with different attacks on examples with ground truth label 2}
%    \end{subfigure}
%    \begin{subfigure}
%        \includegraphics[width=.4\linewidth]{figures/mnist/attack_trans_coeff_label_4.png}
%%        \caption{Correlation of transferability generated with different attacks on examples with ground truth label 2}
%    \end{subfigure}
%    \begin{subfigure}
%        \includegraphics[width=.4\linewidth]{figures/mnist/attack_trans_coeff_label_5.png}
%%        \caption{Correlation of transferability generated with different attacks on examples with ground truth label 2}
%    \end{subfigure}
%    \begin{subfigure}
%        \includegraphics[width=.4\linewidth]{figures/mnist/attack_trans_coeff_label_6.png}
%%        \caption{Correlation of transferability generated with different attacks on examples with ground truth label 2}
%    \end{subfigure}
%    \begin{subfigure}
%        \includegraphics[width=.4\linewidth]{figures/mnist/attack_trans_coeff_label_7.png}
%%        \caption{Correlation of transferability generated with different attacks on examples with ground truth label 2}
%    \end{subfigure}
%    \begin{subfigure}
%        \includegraphics[width=.4\linewidth]{figures/mnist/attack_trans_coeff_label_8.png}
%%        \caption{Correlation of transferability generated with different attacks on examples with ground truth label 2}
%    \end{subfigure}
%    \begin{subfigure}
%        \includegraphics[width=.4\linewidth]{figures/mnist/attack_trans_coeff_label_9.png}
%%        \caption{Correlation of transferability generated with different attacks on examples with ground truth label 2}
%    \end{subfigure}
%    \caption{Correlation of transferability generated on examples from different classes with different attacks}
%    \label{fig:attack_trans_coeff_label}
%\end{figure}

\begin{figure}
\centering
\subcaptionbox{Label 0}{
    \includegraphics[width=0.4\linewidth]{figures/mnist/attack_trans_coeff_label_0.png}
}
\hfill
\subcaptionbox{Label 1}{
    \includegraphics[width=0.4\linewidth]{figures/mnist/attack_trans_coeff_label_1.png}}%
\hfill
\subcaptionbox{Label 2}{
    \includegraphics[width=0.4\linewidth]{figures/mnist/attack_trans_coeff_label_2.png}}%
\hfill
\subcaptionbox{Label 3}{
    \includegraphics[width=0.4\linewidth]{figures/mnist/attack_trans_coeff_label_3.png}}%
\hfill
\subcaptionbox{Label 4}{
    \includegraphics[width=0.4\linewidth]{figures/mnist/attack_trans_coeff_label_4.png}
}
\hfill
\subcaptionbox{Label 5}{
    \includegraphics[width=0.4\linewidth]{figures/mnist/attack_trans_coeff_label_5.png}}%
\hfill
\subcaptionbox{Label 6}{
    \includegraphics[width=0.4\linewidth]{figures/mnist/attack_trans_coeff_label_6.png}}%
\hfill
\subcaptionbox{Label 7}{
    \includegraphics[width=0.4\linewidth]{figures/mnist/attack_trans_coeff_label_7.png}}%
\hfill
\subcaptionbox{Label 8}{
    \includegraphics[width=0.4\linewidth]{figures/mnist/attack_trans_coeff_label_8.png}}%
\hfill
\subcaptionbox{Label 9}{
    \includegraphics[width=0.4\linewidth]{figures/mnist/attack_trans_coeff_label_9.png}}%
\caption{Correlation of transferability generated on examples from different classes with different attacks}
\label{fig:attack_trans_coeff_label}
\end{figure}

To summarize our results about transferability rankings, we proved the following assumptions:
\begin{itemize}
    \item Transferability ranking is similar attack-wise no matter the ground truth label for target example is,
    attackers can use the one generated with one-step fast attack algorithms as the approximation for other
    iteration-based or optimization-based attacks.
    \item Transferability ranking is similar dataset-wise, attackers can use transferability ranking generated on a set
    with fewer examples as the approximation to generate adversarial examples on a larger set of examples.
    \item Transferability ranking is not similar label-wise, it's not the best strategy for attackers to perform our
    transferability-based adaptive attack ignoring the difference.
\end{itemize}

However, as all of attack algorithm used to evaluate the transferability ranking is all gradient based, the high
correlation only indicates that those ensemble members have different robustness towards gradient-based attacks and
we leave the evaluation for decision-based or score-based attacks for future work.

During our experiment, time cost for transferability ranking of 72 ensemble members as in~\cite{athena} under FGSM
attack on one example is around 4 minutes, and it'll take longer for iteration-based or optimization-based attacks
like PGD, C\&W l2 and DeepFool.
By approximating transferability ranking on certain example with the pre-generated one on randomly drawn 100 examples,
it speeds up the adaptive attack procedure and also improves the success rate for our adaptive attacks.
Moreover, as there's only a few changes among the transferability ranking under different attack, it is possible for us
to construct a distilled ensemble based on transferability ranking under FGSM which is able to be robust towards
other attack algorithms.

\subsection{Adaptive Attacks against Ensemble Defense}\label{subsec:adaptive-attacks-against-ensemble-defense}
As mentioned in~\ref{subsec:adaptive-attack}, we performed three sets of adaptive attacks on the ensemble from~
\ref{meng2020ensembles}, with their white-box/gray-box attack as baseline, the results are
in~\ref{tab:mnist_attack_result}.

For \textit{Original}, \textit{label-wise TR}, \textit{overall TR} setting, we evaluate them on the whole test dataset
with 5000 examples with their transferability ranking mentioned in~\ref{subsec:transferability-results}.
For \textit{Individual TR} setting, we evaluate it on a small dataset with 100 examples since it's expensive to generate
transferability ranking for every example with different attacks.
Budget dissimilarity for our adaptive attack is set to 0.1.

From Table.~\ref{tab:mnist_attack_result}, it is obvious that the classification accuracy is the lowest under adaptive
attack with FGSM\@.
This result is in line with~\cite{BIM}, where they took photos of printed generated adversarial images as input of
target classifier.
We also adopt their explanation for this as FGSM is a one-step algorithm while iterative based attack algorithms will
update adversarial perturbations for many iterations and eventually generates more subtle perturbations.

Our results in Table.~\ref{tab:mnist_attack_result} also indicates adaptive attack with \textit{Overall TR} on test
dataset is not as effective as adaptive attack with \textit{Label-wise TR}, this further proves our assumption about
robustness of classifiers is different as ground truth label of example differs.
Also, as classification accuracy of ensemble under adaptive attacks with FGSM, C\&W or DeepFool using \textit{label-wise TR}
drops 30\% to 40\% compared to the one using \textit{overall TR}, while classification accuracy of ensemble under adaptive
attack with PGD in \textit{overall TR} and \textit{label-wise TR} are almost the same for only 4\% to 5\% performance drop.
We think the reason is that number of iterations for PGD is so high that generated adversarial perturbation is subtle
and destroyed during transformations.

Compare the result in Table.~\ref{tab:mnist_attack_result} under \textit{original} and \textit{Transformed},
we can see that adversarial examples generated on transformed input are more aggressive than those
generated on original input even without knowledge about transferability ranking of ensemble members.
Also, compare the performance under \textit{Transformed} and \textit{Overall TR}, it is clear that transferability ranking
based adaptive attack improves the success rate of adversary.

However, for adaptive attack with C\&W or DeepFool, their success rates are higher under \textit{Label-wise TR} compared
to the one under \textit{Individual TR}.
We looked into for the explanation and found out that for FGSM and PGD adaptive attacks, it takes fewer iterations under
\textit{Label-wise TR} while for C\&W and DeepFool adaptive attacks, it takes more iterations for adversary to exceed the
budget limitation.
As mentioned in sec.~\ref{subsec:ensemble-defense}, input transformation is more destructive on subtle perturbations and
the more iteration an adversary runs, the more delicate its perturbation is and this explains why C\&W and DeepFool
adaptive attacks have better performance under \textit{Label-wise TR} than on \textit{Individual TR}.

Also not surprisingly, as pointed out in Table.~\ref{tab:mnist_attack_result}, our adaptive attack generated with FGSM using
\textit{individual TR} brings down the accuracy of original ensemble with 72 transformations from 99.68\% to 33\%.
This means that in actual attack scenarios, where adversaries are always example-specific, generating the transferability
ranking on this particular example and perform our adaptive attack can have around 67\% chance to successfully
fool an ensemble with 72 ensemble members.

\subsection{Effectiveness of Weak Classifiers in Ensemble}\label{subsec:effectiveness-of-weak-classifiers-in-ensemble}
\begin{table}[t]
\centering
\caption{Classification Accuracy of ensembles with different number of members on benign MNIST examples}
\label{tab:limited_benign_accu}
\resizebox{\columnwidth}{!}{%
\begin{tabular}{|c|l|l|l|l|l|}
\hline
\multicolumn{1}{|l|}{} & \multicolumn{1}{c|}{\textbf{RD}} & \multicolumn{1}{c|}{\textbf{MV}} & \multicolumn{1}{c|}{\textbf{T2MV}} & \multicolumn{1}{c|}{\textbf{AP}} & \multicolumn{1}{c|}{\textbf{AL}} \\ \hline
\textbf{\begin{tabular}[c]{@{}c@{}}ensemble\\ of\\ 72 models\end{tabular}} & 0.9958 & 0.9968 & 0.9945 & 0.9968 & 0.9968 \\ \hline
\textbf{\begin{tabular}[c]{@{}c@{}}ensemble\\ of\\ 20 models\end{tabular}} & 0.9926 & 0.9968 & 0.966 & 0.9966 & 0.9972 \\ \hline
\textbf{\begin{tabular}[c]{@{}c@{}}ensemble\\ of\\ 10 models\end{tabular}} & 0.992 & 0.9968 & 0.9458 & 0.9968 & 0.9966 \\ \hline
\textbf{\begin{tabular}[c]{@{}c@{}}ensemble\\ of\\ 5 models\end{tabular}} & 0.9926 & 0.9962 & 0.9114 & 0.9964 & 0.9972 \\ \hline
\end{tabular}%
}
\end{table}
To make our ensemble more robust, we may need to select our ensemble members to ensure there's no shortage within
them.
Our selection is based on transferability, we select $N$ ensemble members with the lowest transferability ranking and
construct a new ensemble model with them.
We evaluate the classification accuracy of ensembles with different number of ensemble members selected by our
transferability ranking based selection on benign examples in Table.~\ref{tab:limited_benign_accu}.
It is clear that for classification task on MNIST, distilled ensemble with 5 ensemble members can have great performance
for benign examples and there's no trading benign performance for robustness in our ensemble distillation method.

Also, we test the classification accuracy of distilled ensemble with 10 members under our adaptive attack using 
\textit{Overall TR} in Table.~\ref{tab:limited_adv_accu}.
\begin{table}[b]
\centering
\caption{Classification Accuracy of ensembles with 10 members under adaptive attack using Overall TR on MNIST}
\label{tab:limited_adv_accu}
\resizebox{\columnwidth}{!}{%
\begin{tabular}{|c|l|l|l|l|l|}
\hline
\multicolumn{1}{|l|}{} & \multicolumn{1}{c|}{\textbf{RD}} & \multicolumn{1}{c|}{\textbf{MV}} & \multicolumn{1}{c|}{\textbf{T2MV}} & \multicolumn{1}{c|}{\textbf{AP}} & \multicolumn{1}{c|}{\textbf{AL}} \\ \hline
\textbf{FGSM} & 0.9908 & 0.9954 & 0.9892 & 0.9954 & 0.9954 \\ \hline
\textbf{PGD} & 0.9912 & 0.9966 & 0.9918 & 0.9966 & 0.997 \\ \hline
\textbf{C\&W} & 0.9872 & 0.9934 & 0.9908 & 0.9932 & 0.9938 \\ \hline
\textbf{DeepFool} & 0.9222 & 0.9948 & 0.9928 & 0.9948 & 0.9948 \\ \hline
\end{tabular}%
}
\end{table}
Compared the result of 10-member ensemble and the original \textit{Athena} ensemble under the same adaptive attack,
the classification accuracy increases from 60\% to 99.54\%, proving high robustness for this distilled ensemble.

With improved robustness against our adaptive attacks and no performance drop on benign data points, it is proved
that those classifiers with high transferability ranking is not helping the ensemble be robust but be less robust.
This can be explained that as the transferability ranking is a nature of ensemble member (weak classifier) and
diversity of ensemble is directly related to the robustness.
Hence, for adversarial data points, the higher the transferability ranking of a model is, the more models that the
model is similar to, and the lower diversity, leading to less robust towards adversarial examples;
for benign data point, those weak defences increase the redundancy of ensemble and its performance on benign examples
can be improved under certain ensemble strategies but as the performance of single weak becomes better, the ensemble
requires less but distilled ensemble members to be both accurate and robust.

==> transferability-based-adaptive-attack-and-defense.tex <==
\subsection{Adaptive Attack}\label{subsec:adaptive-attack}
Authors of~\cite{Carlini} evaluated 13 defense methods towards adversarial examples proposed in the year of 2019 and
performed adaptive attacks on them to have their robustness under the worst-case scenario.
Unfortunately, all of these 13 defense methods in~\cite{Carlini} fail to make the correct prediction on adversarial
examples generated by their corresponding adaptive attack.
Moreover, for most of the adaptive attacks proposed in~\cite{Carlini}, they just adopt an iterative attack algorithm like
PGD and apply it for several random starts with larger number of epochs for each start.
This reminds us to set up our defense method against adversaries with more budget on both computational power and time to
simulate the performance of our defended ensemble under the worst-case scenario.

In this paper, we proposed a transferability-based adaptive attack and distillation method for ensemble as a defense.
Unlike adaptive attacks in~\cite{Carlini}, our adaptive attack comes from Liebig's law of the minimum in agricultural
science, it originally states that growth is dictated not by total resources available, but by the scarcest resources.
In our case, we treat the robustness of ensemble as the growth while resources are transferability of adversarial
examples targeting on different ensemble members.
It may be hard for adversaries to find adversarial example to break the defense of our ensemble but as mentioned in
section~\ref{subsec:evasion-attack}, it only requires adversaries to find the overlapping area bounded by the decision
boundaries of majority of ensemble members and the ground truth data distribution to successfully generate an adversarial
example that fools the ensemble model.

With this in mind, the most efficient way for adversaries becomes find the most representative ensemble member whose decision
boundaries have the largest overlapping area with ground truth data distribution such that searching in this area can
definitely leads to a successful adversarial example.
Here in this paper, we use the transferability of adversarial examples targeting on ensemble member as the numerical
expression of how this ensemble member is representative for all the ensemble members, we refer the ranking of
transferability of adversarial examples generated on every ensemble member as transferability ranking.

We tested three ways to find the most representative ensemble member and performed adaptive attack with them accordingly:
transferability ranking of all ensemble members on a specific example (individual ranking);
average transferability ranking of all ensemble members on a specific set of examples from all classes (average ranking);
average transferability ranking of all ensemble members on a specific set of examples from the same class (label ranking).
We'll describe their implementations in detail in following sections.

In line with the budge setting in~\cite{meng2020ensembles}, we adopt their normalized $l_2$ dissimilarity as the budget
function of our adaptive attacks in Eq.~\ref{eq:dissimilarity}
\begin{equation}
    dissimilarity(x_0, x_{adv}) = \frac{||x_0-x_{adv}||_2}{||x_0||_2}
    \label{eq:dissimilarity}
\end{equation}
Also, since the goal for setting budget is to keep the generated adversarial perturbation unnoticeable and able to be
classified correctly by a golden-standard classifier, we'll calculate the dissimilarity between adversarial example and
benign example after corresponding transformation.
The reason we perform it on transformed examples is that examples after transformations can still be recognized correctly
by human eyes and they should be set as the baseline for dissimilarity comparison.

\subsubsection{Adaptive Attack on transformed input}
\label{subsubsec:why on transformed input}
As mentioned in~\ref{subsec:ensemble-defense}, input transformation is a strong defense method by destroying some subtle
perturbations.
Hence, if the adversary conduct attacks on examples without transformation, adversarial perturbations from the non-
transformed domain may not be able to be kept in transformed domain and lower down the success rate of attacks.
By generating adversarial perturbations on transformed input, adversary bypasses the part of transformation barrier.
However, transformations still play their role of defender as it is still required for adversarial examples to be fed
into ensemble model after transformations during inference time.
Effectiveness of generating perturbations on transformed inputs will be demonstrated in section~\ref{sec:experiment}.

Besides, since adversarial examples are generated on transformed images and transformations are applied to adversarial
images before feeding into ensemble model during inference time in our case, once transformations involving orientation
or position shift of the main figure, it may lead to a transformation of shift images to its bottom right applied on an
an adversarial example generated on image shifted to bottom right during attack.
Hence, we implemented a reset function to reset possible position or orientation shifts during attack procedure and for
certain non-invertible transformations like swirl, we won't select them as our target ensemble member during attack.

\subsubsection{Transferability ranking generated for every individual example (Individual TR)}
\label{subsubsec:individual-ranking-based}
The algorithm of adaptive attack based on transferability ranking on specific example is shown in
Algorithm~\ref{alg:attack-algorithm}.
It consists of two main parts: generate the transferability ranking for every target sample and perform adversarial
attack on the model selected by transferability in a descending order.
Compared to the white-box or gray-box attacks mentioned in~\cite{meng2020ensembles},
the time complexity of our adaptive attack is still $ O(m^2) $ but however, as time complexity for transferability
ranking evaluation part is also $O(m^2)$, the actual time cost for our adaptive attack using individual ranking is much
higher compared to the white-box evaluation in~\ref{meng2020ensembles}.

\subsubsection{Average transferability ranking generated on 100 random chosen examples (Overall TR)}
\label{subsubsec:average-ranking-over-all-examples}
As in Algorithm~\ref{alg:attack-algorithm}, one needs to generate transferability ranking by iterate attacking through all the
ensemble members twice, which makes the time complexity of transferability ranking to $O(n^2)$.
In our experiments, it takes more than 4 minutes to finish one transferability ranking of one example for FGSM
attack, and the time cost for iteration-based or optimization-based methods can only be higher.

To accelerate the attacking procedure, we tried to use transferability ranking generated on less examples or faster
attack algorithms to mimic the overall performance.
In \textit{Overall TR} setting, we take the average transferability ranking on 100 random chosen examples with FGSM
attack as the overall transferability ranking among all examples under all attacks in our experiments
(FGSM, PGD, C\&W $l_2$, DeepFool).
In following experiments, we'll show that the transferability ranking is similar for different attacks and also for
different sizes of examples used to generated the transferability ranking.

\subsubsection{Average transferability ranking generated for every class in 100 random chosen examples (Label-wise TR)}
\label{subsubsec:average-ranking-over-classes}
According to~\cite{liu2016delving}, the transferability of adversarial examples generated on data belongs to different
classes may differs.
Hence, using a transferability ranking generated on a small set of examples from different classes as the overall
transferability ranking for all examples might not be accurate.

In this attack scenario, we generate the transferability ranking on the same randomly chosen examples as in section~
\ref{subsubsec:average-ranking-over-all-examples} but according to their ground truth labels, i.e., one transferability
ranking for one class of examples.

\subsection{Defense}\label{subsec:defense}
The methodology of our adaptive attack comes from the idea of Liebig's law of the minimum, but in our case, we can select
our ensemble members to achieve more robust towards adversarial examples while in the original context of Liebig's law
of the minimum, those resources are all essential and cannot be further optimized.
However, in our case of ensemble defense, we can create a new ensemble with less but necessary ensemble members with
guaranteed diversity.

As mentioned in section~\ref{subsec:evasion-attack}, diversity of ensemble members guarantee the robustness of the whole
ensemble model.
In our ensemble of 72 models trained on differently transformed examples, diversity of ensemble members can be
approximated by the transferability of adversarial examples trained on this particular ensemble member as we referred as
transferability ranking in previous sections.
Hence, we select $N$ ensemble members from the lowest transferability to guarantee the diversity of ensemble.

The transferability ranking used for selection is the one generated on the randomly chosen 100 examples with FGSM attack
since it's neither data-dependent nor attack-dependent and it's highly similar to transferability ranking generated on
a larger set of examples and also those generated with other attack algorithms as indicated in section~
\ref{subsec:transferability-results}.

\begin{algorithm}[t]
    \caption{Adaptive Attack under white box setting}
    \label{alg:attack-algorithm}
    \KwInput{x, y, attacker, maximum dissimilarity}
    \KwOutput{adversarial examples $ x_{adv} $}
    \ForEach{ensemble member $ \in $ ensemble members}{
    $x_{adv} \leftarrow attacker.attack(x)$ \\
    $count$ $\leftarrow$ EMPTY DICTIONARY \\
    \ForEach{ensemble member $ \in $ ensemble members}{
    \If{ensemble member.predict(transform$ target(x_{adv}$, ensemble member)) $\neq$ y}{
    count[ensemble member] $\leftarrow$ count[ensemble member] + 1
    }
        }
    }
    $ S_{fooled} \leftarrow  $ EMPTY SET \\
    $ S_{candidates} \leftarrow  $ sort by values(count) \\
    $x_{adv} \leftarrow $ x  \\
    \While{True}{
    target $\leftarrow$ pick target($S_{cand}$) \\
    $ x_{ori} \leftarrow $ transformation.transform($x$, target)  \\
    $x_{trans} \leftarrow  $ transformation.transform($x_{adv}$, target) \\
    $x_{tmp}$ $\leftarrow$ attacker.attack($x_{trans}$) \\
    dis $\leftarrow$ normalized $l_2$ norm($x_{tmp}, x_{ori}$) \\
    \If{dis $ \geq $ maximum dissimilarity}{
    break
    }
        $ x_{adv} \leftarrow reset(x_{tmp}) $ \\
        \ForEach{candidate $ \in $ $ S_{candidates} $}{
        \If{candidate.predict(transform($ x_{adv}$, candidate))}{
        $S_{candidates}$.remove(candidate) \\
        $S_{fooled}$.add(candidate)
        }
            }
    }
        return $x_{adv}$

\end{algorithm}

